Comparative Analysis and Behavioral Modelling of Power Amplifiers in FR3

Power amplifier (PA) nonlinearity is a critical transmitter impairment in the upper mid-band (7 GHz to 24 GHz), designated as Frequency Range 3 (FR3) in emerging 6G standardisation. The 3GPP PA model baseline, TR 38.803 Annex A, was derived from 2.1 GHz and 28 GHz measurements and has not been revisited yet for FR3 standards work. This paper addresses that gap with characterisation measurements of multiple PA devices-under-test (DUTs), driven into gain compression in the 7 GHz and 15 GHz bands with 100 MHz and 200 MHz bandwidth. Memoryless polynomial and Generalized Memory Polynomial (GMP) behavioral models are extracted by least-squares regression and compared with 3GPP models spanning FR1 and FR2. The GaN PA DUT is modelled best at a higher nonlinear order and shows markedly stronger phase distortion than the wideband PA. The memory terms of the GMP model measurably improve the Normalized Mean Square Error (NMSE) at all operating points. An orthogonal frequency-division multiplexing (OFDM) ambiguity function analysis from the Integrated Sensing and Communication (ISAC) literature, using the extracted models, illustrates how PA compression raises the sidelobe floor of the sensing response. These results provide a reference for PA impairment modelling in FR3, directly applicable to ISAC system design. All model coefficients and measurement data are publicly available [1].

==> tables/tab_coefficients.tex <==
% generated by matlab/s06_nmse_table.m -- do not edit by hand
    $a_{1}$ & $0.433677{-}0.0861185j$ & $0.991353{+}0.00156095j$ & $0.461264{+}0.0013169j$ & $0.518208{+}0.00144462j$ & $1.55834{+}0.0378682j$ \\
    $a_{3}$ & $-0.611734{+}0.697125j$ & $-0.377013{-}0.0043936j$ & $-0.0766644{-}0.00409608j$ & $-0.111147{-}0.00481689j$ & $-0.229803{-}0.117651j$ \\
    $a_{5}$ & $1.65269{-}2.22394j$ & $0.191939{-}0.00142087j$ & -- & -- & -- \\
    $a_{7}$ & $-2.85069{+}3.95772j$ & -- & -- & -- & -- \\
    $a_{9}$ & $2.55906{-}3.56465j$ & -- & -- & -- & -- \\
    $a_{11}$ & $-0.906097{+}1.25627j$ & -- & -- & -- & -- \\


==> tables/tab_models_measured.tex <==
% generated by matlab/s06_nmse_table.m -- do not edit by hand
    GaN PA & 8\,GHz, 100\,MHz & 11 / 11 & 6 / 64 & $-39.4$ & $-40.8$ & $-1.4$ \\
    TLPA & 7.225\,GHz, 200\,MHz & 5 / 5 & 3 / 27 & $-29.5$ & $-31.7$ & $-2.2$ \\
    TLPA & 15\,GHz, 100\,MHz & 3 / 5 & 2 / 27 & $-31.8$ & $-34.7$ & $-2.9$ \\
    TLPA & 15\,GHz, 200\,MHz & 3 / 5 & 2 / 27 & $-28.1$ & $-32.7$ & $-4.6$ \\
    GaAs LNA & 15\,GHz, 100\,MHz & 3 / 7 & 2 / 34 & $-29.2$ & $-31.6$ & $-2.4$ \\


==> tables/tab_same_order.tex <==
% generated by matlab/s06_nmse_table.m -- do not edit by hand
    GaN PA & 8/100 & 11 & 6 / $-39.4$ & 42 / $-40.4$ & 64 / $-40.8$ \\
    TLPA & 7.225/200 & 5 & 3 / $-29.5$ & 21 / $-31.5$ & 27 / $-31.7$ \\
    TLPA & 15/100 & 3 & 2 / $-31.8$ & 14 / $-34.4$ & 18 / $-34.6$ \\
    TLPA & 15/200 & 3 & 2 / $-28.1$ & 14 / $-32.2$ & 18 / $-32.6$ \\
    GaAs LNA & 15/100 & 3 & 2 / $-29.2$ & 14 / $-31.4$ & 14 / $-31.4$ \\

